Towards Transparent and Explainable Attention Models

Recent studies on interpretability of attention distributions have led to notions of faithful and plausible explanations for a model's predictions. Attention distributions can be considered a faithful explanation if a higher attention weight implies a greater impact on the model's prediction. They can be considered a plausible explanation if they provide a human-understandable justification for the model's predictions. In this work, we first explain why current attention mechanisms in LSTM based encoders can neither provide a faithful nor a plausible explanation of the model's predictions. We observe that in LSTM based encoders the hidden representations at different time-steps are very similar to each other (high conicity) and attention weights in these situations do not carry much meaning because even a random permutation of the attention weights does not affect the model's predictions. Based on experiments on a wide variety of tasks and datasets, we observe attention distributions often attribute the model's predictions to unimportant words such as punctuation and fail to offer a plausible explanation for the predictions. To make attention mechanisms more faithful and plausible, we propose a modified LSTM cell with a diversity-driven training objective that ensures that the hidden representations learned at different time steps are diverse. We show that the resulting attention distributions offer more transparency as they (i) provide a more precise importance ranking of the hidden states (ii) are better indicative of words important for the model's predictions (iii) correlate better with gradient-based attribution methods. Human evaluations indicate that the attention distributions learned by our model offer a plausible explanation of the model's predictions. Our code has been made publicly available at https://github.com/akashkm99/Interpretable-Attention

==> experiments_explainability.tex <==
%\section{Experiments on Explainability}

% The diversity LSTM and standard LSTM models were run on different tasks to juxtapose their attention distributions for volunteers to rate, to validate our contention that diversifying the attention distributions correlates with an increase in human interpretability of attention weights. 


% The role of the volunteer was to choose the better heatmap/explanation that helped explain the models decision. . For each criteria the person was given 4 options to choose from, a) heatmap 1 b) heatmap 2 c) Same-Bad d) Same-Good, where same-bad and same-good indicate that both models heatmaps were equally bad or good in the given criteria. Each sample was rated by 3 different raters and the inter annotation agreement coefficient was computed for all datasets, using Fleiss coefficient (cite here).

% The fleiss inter-annotator agreement score overall ranged between 0.288 to 0.442 with a mean of 0.376, indicating that there was fair to moderate agreement between raters choices. Overall, in all criteria, the diverse model with weight 0.5 was selected substantially more than the standard model counterpart. The difference in averages (shown in ) between the models for any criteria in any dataset never went below 13.63 (in overall precise, SNLI), in favor of the diversity model. 


% We can see that in the “Entailment” and “Neutral” output classes of the SNLI dataset, the Diversity model is equally preferred and sometimes even less preferred to the Standard model, but dominates in the “Contradiction” class. This anomaly is due unique difference in nature of the “Entailment” and “Neutral” tasks, compared to the other tasks we have seen so far in other datasets. The idea is that these two tasks expect or only require a narrow span of attention on a few words, which the diversity LSTM does not generally prefer doing.

% In most of the instances that the Diversity LSTM fails, the general trend can be shown by the following example in the entailment task, There is a man and Man holding torch of fire. The two statements entail each other (given the first statement is true, the other support) because of the presence of the entity “man” in both sentences. In the second statement, the information after the word “man” is irrelevant in contributing to the entailment relation between the two statements. In this case the standard model gives most of its attention to “man” and the diversity model incorrectly tries to diversify its attention and avoids giving attention to “man”, leading to raters preferring the standard model. Thus this particular task is slightly biased towards being less interpretable to diversified attention and favours the narrow attentions of the standard model. The same reasoning applies for the neutrality task, in which attention is expected to be given to a narrow span of words. This type of bias does not occur generally in most tasks.

==> table_correlations.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\if 0 
\begin{table*}[]
\centering
% \resizebox{0.95\textwidth}{!}{
\scriptsize{
\begin{tabular}{l|cc|cc|cc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Gradients\\ (Mean $\pm$ Std.)\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Integrated Gradients\\ (Mean $\pm$ Std.)\end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Rationales\\ (Attention given / Length)\end{tabular}}} \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{Vanilla}                    & \multicolumn{1}{c|}{Diversity}                    & \multicolumn{1}{c|}{Vanilla}                          & \multicolumn{1}{c|}{Diversity}                         & \multicolumn{1}{c|}{Vanilla}                       & \multicolumn{1}{c}{Diversity}                       \\ \hline
\multicolumn{7}{c}{\textbf{Text Classification}}                                                                                                                                                                                                                                                                                                                                         \\ \hline
SST                                                     & 0.712  $\pm$ 0.216                              & 0.831 $\pm$ 0.197                                 & 0.629 $\pm$ 0.246                                     & 0.798 $\pm$ 0.224                                      & 0.348 / 0.240                                        & 0.624 / 0.175                                          \\
IMDB                                                    & 0.805 $\pm$ 0.077                               & 0.898 $\pm$ 0.040                                 & 0.682 $\pm$ 0.095                                     & 0.782 $\pm$ 0.077                                      & 0.472 / 0.217                                        & 0.761 / 0.169                                          \\
Yelp                                                    & 0.553 $\pm$ 0.169                               & 0.795 $\pm$ 0.122                                 & 0.408 $\pm$ 0.191                                     & 0.795 $\pm$ 0.148                                      & 0.438 / 0.173                                        & 0.574 / 0.160                                          \\
Amazon                                                  & 0.437 $\pm$ 0.198                               & 0.772 $\pm$ 0.145                                 &                                                       &                                                        & 0.346 / 0.162                                        & 0.396 / 0.240                                          \\
Anemia                                                  & 0.635 $\pm$ 0.129                               & 0.729 $\pm$ 0.101                                 & 0.437 $\pm$ 0.157                                     & 0.661 $\pm$ 0.118                                      & 0.611  /  0.192                                        & 0.739  /  0.237                                          \\
Diabetes                                                & 0.654 $\pm$ 0.155                               & 0.766 $\pm$ 0.133                                 & 0.553 $\pm$ 0.147                                     & 0.691 $\pm$ 0.183                                      & 0.742 / 0.458                                        & 0.825 / 0.354                                          \\
20News                                                  & 0.727 $\pm$ 0.280                               & 0.964 $\pm$ 0.080                                 & 0.659 $\pm$ 0.320                                     & 0.671 $\pm$ 0.112                                      & 0.627 / 0.215                                        & 0.884 / 0.173                                          \\
Tweets                                                  & 0.657 $\pm$ 0.244                               & 0.800 $\pm$ 0.210                                 & 0.567 $\pm$ 0.258                                     & 0.744 $\pm$ 0.222                                      & 0.284 / 0.225                                        & 0.764 / 0.306                                           \\ \hline
\multicolumn{7}{c}{\textbf{Natural Language Inference}}                                                                                                                                                                                                                                                                                                                                  \\ \hline
SNLI                                                    & 0.580 $\pm$ 0.331                               & 0.510 $\pm$ 0.354                                 & 0.381 $\pm$ 0.406                                     & 0.269 $\pm$ 0.399                                      & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                                 \\ \hline
\multicolumn{7}{c}{\textbf{Paraphrase Detection}}                                                                                                                                                                                                                                                                                                                                        \\ \hline
QQP                                                     & 0.195 $\pm$ 0.344                               & 0.580 $\pm$ 0.315                                 & -0.061 $\pm$ 0.344                                    & 0.216 $\pm$ 0.36                                       & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                                 \\ \hline
\multicolumn{7}{c}{\textbf{Question Answering}}                                                                                                                                                                                                                                                                                                                                          \\ \hline
Babi 1                                                  & 0.561 $\pm$ 0.343                               & 0.916 $\pm$ 0.104                                 & 0.331 $\pm$ 0.379                                     & 0.916 $\pm$ 0.104                                      & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                                 \\
Babi 2                                                  & 0.167 $\pm$ 0.237                               & 0.707 $\pm$ 0.139                                 & 0.055 $\pm$ 0.222                                     & 0.757 $\pm$ 0.109                                      & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                                 \\
Babi 3                                                  & 0.398 $\pm$ 0.240                               & 0.677 $\pm$ 0.199                                 & -0.010 $\pm$ 0.084                                    & 0.475 $\pm$ 0.254                                      & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                                 \\
CNN                                                     & 0.580 $\pm$ 0.250                               & 0.758 $\pm$ 0.205                                 & 0.453 $\pm$ 0.284                                     & 0.661 $\pm$ 0.238                                      & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                                
\end{tabular}}
\caption{Comparison of Attention weights with Gradient-based feature importance methods and Generated rationales. Column 2 and 3 reports the Mean and Standard Deviation of Pearson correlations between Attention weights and Gradients/Integrated Gradients in Vanilla and Diversity LSTM models. Column 4 reports the mean Attention given to the generated rationales and the mean length of the rationales (in fraction).}
\label{tab:correlations}
\end{table*}
\fi

\begin{table}[]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{|l|cc|cc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Gradients\\ (Mean $\pm$ Std.)\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Integrated Gradients\\ (Mean $\pm$ Std.)\end{tabular}}}  \\ \cline{2-5} 

\multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{Vanilla}                    & \multicolumn{1}{c|}{Diversity}                    & \multicolumn{1}{c|}{Vanilla}                          & \multicolumn{1}{c|}{Diversity}  \\ \hline
\multicolumn{5}{c}{\textbf{Text Classification}}                                                                                                                                                                                                                                                                                                                                         \\ \hline
SST                                                     & 0.71 $\pm$0.22                              & 0.83 $\pm$ 0.20                               & 0.63 $\pm$ 0.25                                     & 0.80 $\pm$ 0.22                                                         \\
IMDB                                                    & 0.81 $\pm$ 0.08                               & 0.90 $\pm$ 0.04                                 & 0.68 $\pm$ 0.09                                     & 0.78 $\pm$ 0.08                                                                   \\
Yelp                                                    & 0.55 $\pm$ 0.17                               & 0.80 $\pm$ 0.12                                 & 0.41 $\pm$ 0.19                                    & 0.80 $\pm$ 0.15                                                             \\
Amazon                                                  & 0.44 $\pm$ 0.20                               & 0.77 $\pm$ 0.15                                 & 0.23 $\pm$ 0.25                                                     & 0.69  $\pm$ 0.17                                                                                 \\
Anemia                                                  & 0.64 $\pm$ 0.13                               & 0.73 $\pm$ 0.10                                 & 0.44 $\pm$ 0.16                                     & 0.66 $\pm$ 0.12                                                                         \\
Diabetes                                                & 0.65 $\pm$ 0.15                               & 0.77 $\pm$ 0.13                                 & 0.55 $\pm$ 0.15                                     & 0.69 $\pm$ 0.18                                                                    \\
20News                                                  & 0.73 $\pm$ 0.28                               & 0.96 $\pm$ 0.08                                 & 0.65 $\pm$ 0.32                                     & 0.67 $\pm$ 0.11                                                                    \\
Tweets                                                  & 0.65 $\pm$ 0.24                               & 0.80 $\pm$ 0.21                             & 0.57 $\pm$ 0.26                                     & 0.74 $\pm$ 0.22                                                              \\ \hline
\multicolumn{5}{c}{\textbf{Natural Language Inference}}                                                                                                                                                                                                                                                                                                                                  \\ \hline
SNLI                                                    & 0.58 $\pm$ 0.33                               & 0.51 $\pm$ 0.35                                 & 0.38 $\pm$ 0.41                                     & 0.27 $\pm$ 0.40                                                                 \\ \hline
\multicolumn{5}{c}{\textbf{Paraphrase Detection}}                                                                                                                                                                                                                                                                                                                                        \\ \hline
QQP                                                     & 0.20 $\pm$ 0.34                               & 0.58 $\pm$ 0.32                                 & -0.06 $\pm$ 0.34                                    & 0.22 $\pm$ 0.36                                                                 \\ \hline
\multicolumn{5}{c}{\textbf{Question Answering}}                                                                                                                                                                                                                                                                                                                                          \\ \hline
Babi 1                                                  & 0.56 $\pm$ 0.34                               & 0.92 $\pm$ 0.10                                 & 0.33 $\pm$ 0.38                                     & 0.92 $\pm$ 0.10                                                                \\
Babi 2                                                  & 0.17 $\pm$ 0.24                               & 0.71 $\pm$ 0.14                                 & 0.05 $\pm$ 0.22                                     & 0.76 $\pm$ 0.11                                                                  \\
Babi 3                                                  & 0.40 $\pm$ 0.24                               & 0.68 $\pm$ 0.20                                 & -0.01 $\pm$ 0.08                                    & 0.48 $\pm$ 0.25                                                                \\
CNN                                                     & 0.58 $\pm$ 0.25                               & 0.76 $\pm$ 0.21                                 & 0.45 $\pm$ 0.29                                     & 0.66 $\pm$ 0.24    \\                               \hline                    
\end{tabular}}
\caption{Mean and Std. Dev of Pearson correlations between Attention weights and Gradients/Integrated Gradients in Vanilla and Diversity LSTM models}
\label{tab:correlations}
\end{table}

==> table_lstm_conicity.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
%\resizebox{0.45\textwidth}{!}{
\scriptsize{
\begin{tabular}{l|l|l|l}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{2}{c|}{\textbf{LSTM}} & \textbf{Random} \\ \cline{2-4} 
\multicolumn{1}{c|}{}                                  & Accuracy         & Conicity        & Conicity        \\ \cline{1-4}
\multicolumn{4}{c}{{Text Classification}}                                                             \\ \hline
SST                                                     & 81.79            & 0.68            & 0.25            \\
IMDB                                                    & 89.89            & 0.69            & 0.08            \\
YELP                                                    & 95.60            & 0.53            & 0.14            \\
Amazon                                                  & 93.73            & 0.49            & 0.13            \\
Anemia                                                  & 88.54            & 0.46            & 0.02            \\
Diabetes                                                & 92.31            & 0.61            & 0.02            \\
20News                                                  & 93.55            & 0.77            & 0.13            \\
Tweets                                                  & 87.02            & 0.77            & 0.24            \\ \hline
\multicolumn{4}{c}{{Natural Language Inference}}                                                      \\ \hline
SNLI                                                    & 78.23            & 0.56            & 0.27            \\ \hline
\multicolumn{4}{c}{{Paraphrase Detection}}                                                            \\ \hline
QQP                                                     & 78.74            & 0.59            & 0.30            \\ \hline
\multicolumn{4}{c}{{Question Answering}}                                                              \\ \hline
Babi 1                                                  & 99.10            & 0.56            & 0.19            \\
Babi 2                                                  & 40.10            & 0.48            & 0.12            \\
Babi 3                                                  & 47.70            & 0.43            & 0.07            \\
CNN                                                     & 63.07            & 0.45            & 0.04          \\ \hline 
\end{tabular}}
\caption{Conicity of LSTM hidden states vs Uniformly distributed Vectors:  }
\label{tab:results1}
\end{table}

==> table_predictive_performance.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[bth]
\centering
%\resizebox{0.75\textwidth}{!}{
\scriptsize
\begin{tabular}{|l|ll|ll|ll|l|}
\hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{2}{c|}{\textbf{Vanilla LSTM}}                            & \multicolumn{2}{c|}{\textbf{Diversity LSTM}}                  & \multicolumn{2}{c|}{\textbf{Orthogonal LSTM}}                 & \multicolumn{1}{l|}{\textbf{Random}} \\ \cline{2-8} 
\multicolumn{1}{|l|}{}                                  & \multicolumn{1}{l|}{Accuracy} & \multicolumn{1}{l|}{Conicity} & \multicolumn{1}{l|}{Accuracy} & \multicolumn{1}{l|}{Conicity} & \multicolumn{1}{l|}{Accuracy} & \multicolumn{1}{l|}{Conicity} & \multicolumn{1}{l|}{Conicity}        \\ \hline
\multicolumn{8}{c}{\textbf{Binary Classification}}                                                                                                                                                                                                                                           \\ \hline
SST                                                     & {81.79}                & 0.68                          & 79.57                         & 0.20                          & 79.54                         & 0.28                          & 0.25                                 \\
IMDB                                                    & {89.49}                & 0.69                          & 88.54                         & 0.08                          & 88.71                         & 0.18                          & 0.08                                 \\
Yelp                                                    & 95.60                         & 0.53                          & 95.40                         & 0.06                          & {96.00}                & 0.18                          & 0.14                                 \\
Amazon                                                  & {93.73}                & 0.50                          & 92.90                         & 0.05                          & 93.04                         & 0.16                          & 0.13                                 \\
Anemia                                                  & 88.54                         & 0.46                          & 90.09                         & 0.09                          & {90.17}                & 0.12                          & 0.02                                 \\
Diabetes                                                & {92.31}                & 0.61                          & 91.99                         & 0.08                          & 87.05                         & 0.12                          & 0.02                                 \\
20News                                                  & {93.55}                & 0.77                          & 91.03                         & 0.15                          & 92.15                         & 0.23                          & 0.13                                 \\
Tweets                                                  & 87.02                         & 0.77                          & {87.04}                & 0.24                          & 83.20                         & 0.27                          & 0.24                                 \\ \hline
\multicolumn{8}{c}{\textbf{Natural Language Inference}}                                                                                                                                                                                                                                      \\ \hline
SNLI                                                    & {78.23}                & 0.56                          & 74.16                         & 0.04                          & 76.46                         & 0.27                          & 0.27                                 \\ \hline
\multicolumn{8}{c}{\textbf{Paraphrase Detection}}                                                                                                                                                                                                                                            \\ \hline
QQP                                                     & {78.74}                & 0.59                          & 78.40                         & 0.04                          & 78.61                         & 0.33                          & 0.30                                 \\ \hline
\multicolumn{8}{c}{\textbf{Question Answering}}                                                                                                                                                                                                                                              \\ \hline
bAbI 1                                                  & 99.10                         & 0.56                          & {100.00}               & 0.07                          & 99.90                         & 0.22                          & 0.19                                 \\
bAbI 2                                                  & 40.10                         & 0.48                          & 40.20                         & 0.05                          & {56.10}                & 0.21                          & 0.12                                 \\
bAbI 3                                                  & 47.70                         & 0.43                          & 50.90                         & 0.10                          & {51.20}                & 0.12                          & 0.07                                 \\
CNN                                                     & {63.07}                & 0.45                          & 58.19                         & 0.06                          & 54.30                         & 0.07                          & 0.04                 \\
\hline
\end{tabular}
\caption{Accuracy and Conicity of Vanilla, Diversity  and Orthogonal LSTM on the test dataset}
\label{tab:accuracy_conicity}
\end{table*}
